Multilingual enrichment of disease biomedical ontologies

Translating biomedical ontologies is an important challenge, but doing it manually requires much time and money. We study the possibility to use open-source knowledge bases to translate biomedical ontologies. We focus on two aspects: coverage and quality. We look at the coverage of two biomedical ontologies focusing on diseases with respect to Wikidata for 9 European languages (Czech, Dutch, English, French, German, Italian, Polish, Portuguese and Spanish) for both ontologies, plus Arabic, Chinese and Russian for the second one. We first use direct links between Wikidata and the studied ontologies and then use second-order links by going through other intermediate ontologies. We then compare the quality of the translations obtained thanks to Wikidata with a commercial machine translation tool, here Google Cloud Translation.

==> change.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

      \hline
       & \multicolumn{3}{c|}{$\measureOne{}{}{}$} &\multicolumn{3}{c|}{$\measureTwo{}{}{}$} & \multicolumn{3}{c|}{$\measureThree{}{}{}$} & \multicolumn{3}{c|}{$\measureFour{}{}{}$} \\
      \hline
      Lang & 1st W & 2nd W & GCT & 1st W & 2nd W & GCT & 1st W & 2nd W & GCT & 1st W & 2nd W & GCT\\
      \hline
      EN & \textbf{85.5} & 69.5 & N/A & \textbf{91.5} & 75.6 & N/A & \textbf{84.1} & 61.3 & N/A & \textbf{97.3} & 82.5 & N/A \\
      \hline
      FR & 85.3 (-0.1) & 73.9 & \textbf{90.5} & 87.5 & 75.6 & \textbf{91.2} & 75.7 (-0.5) & 63.4 & \textbf{90.5} & 94.0 (-0.3) & 85.1 & \textbf{98.0} \\
      \hline
      DE & 77.2 (-0.4) & 71.2 & \textbf{84.6} & 80.0 (-0.2) & 72.6 & \textbf{85.8} & 69.1 (-0.6) & 63.2 & \textbf{85.2} & 90.8 (-0.6) & 83.3 & \textbf{96.8} \\
      \hline
      ES & 81.4 (-0.2) & 68.7 & \textbf{94.0} & 84.6 (-0.2) & 71.9 & \textbf{94.6} & 68.9 (-0.5) & 60.7 & \textbf{91.0} & 91.8 (-0.3) & 83.0 & \textbf{99.0} \\
      \hline
      PL & 78.3 (-0.5) & 66.9 & \textbf{84.3} & 82.2 (-0.7) & 68.6 & \textbf{85.6} & 66.7 (-0.7) & 58.6 & \textbf{85.7} & 90.8 (-0.6) & 78.4 & \textbf{96.5} \\
      \hline
      IT & 79.7 (-0.3) & 70.4 & \textbf{90.7} & 82.5 (-0.6) & 72.4 & \textbf{91.7} & 69.3 (-1.0) & 67.0 & \textbf{89.4} & 90.7 (-0.9) & 79.3 & \textbf{98.2} \\
      \hline
      PT & 80.1 (+0.2) & 69.2 & \textbf{87.7} & 82.4 & 70.7 & \textbf{91.1} & 74.1 (-0.4) & 68.8 & \textbf{74.7} & 93.7 (-0.3) & 89.8 & \textbf{95.6} \\
      \hline
      NL & 73.2 (-0.6) & 63.1 & \textbf{86.7} & 75.9 (-0.8) & 64.5 & \textbf{87.3} & 66.2 (-1.1) & 60.7 & \textbf{89.4} & 86.8 (-1.4) & 79.3 & \textbf{98.0} \\
      \hline
      CS & 76.8 (-0.4) & 63.3 & \textbf{86.2} & 79.7 (-0.6) & 65.3 & \textbf{87.8} & 67.8 (-0.7) & 60.1 & \textbf{87.9} & 88.9 (-0.8) & 77.5 & \textbf{97.6} \\
      \hline

\end{tabular}


\begin{tabular}{|l|c|c|}
      \hline
      Language & Cov 1st & New (\%) \\
      \hline
      English & 84.8\% & 195 (1.87\%) \\
      \hline
      French & 47.1\% & 145 (1.39\%) \\
      \hline
      German & 18.1\% & 81 (0.78\%) \\
      \hline
      Spanish & 14.5\% & 68 (0.65\%) \\
      \hline
      Polish & 12.2\% & 61 (0.59\%) \\
      \hline
      Italian & 10.9\% & 56 (0.54\%) \\
      \hline
      Portuguese & 8.5\% & 43 (0.41\%) \\
      \hline
      Dutch & 8.3\% & 42 (0.40\%) \\
      \hline
      Czech & 4.7\% & 19 (0.20\%) \\
      \hline
\end{tabular}
